Cross-Resolution Learning for Face Recognition

Convolutional Neural Networks have reached extremely high performances on the Face Recognition task. Largely used datasets, such as VGGFace2, focus on gender, pose and age variations trying to balance them to achieve better results. However, the fact that images have different resolutions is not usually discussed and resize to 256 pixels before cropping is used. While specific datasets for very low resolution faces have been proposed, less attention has been payed on the task of cross-resolution matching. Such scenarios are of particular interest for forensic and surveillance systems in which it usually happens that a low-resolution probe has to be matched with higher-resolution galleries. While it is always possible to either increase the resolution of the probe image or to reduce the size of the gallery images, to the best of our knowledge an extensive experimentation of cross-resolution matching was missing in the recent deep learning based literature. In the context of low- and cross-resolution Face Recognition, the contributions of our work are: i) we proposed a training method to fine-tune a state-of-the-art model in order to make it able to extract resolution-robust deep features; ii) we tested our models on the benchmark datasets IJB-B/C considering images at both full and low resolutions in order to show the effectiveness of the proposed training algorithm. To the best of our knowledge, this is the first work testing extensively the performance of a FR model in a cross-resolution scenario; iii) we tested our models on the low resolution and low quality datasets QMUL-SurvFace and TinyFace and showed their superior performances, even though we did not train our model on low-resolution faces only and our main focus was cross-resolution; iv) we showed that our approach can be more effective with respect to preprocessing faces with super resolution techniques.

==> subsec/face_datasets/qmul.tex <==
\subsection{QMUL-SurvFace}
The QMUL-SurvFace~\cite{cheng2018surveillance} dataset has 463.5K facial images of 15573 unique identities captured in uncooperative surveillance scenes over wide space and time intervals. Consequently, QMUL-SurvFace represents a true-performance surveillance FR challenge characterised by LR, motion blur, uncontrolled poses, varying occlusion, poor illumination, and background clutters. \autoref{fig:qmul_example} shows a collection of few samples from the dataset.
\begin{figure}[H]
\centering 
\includegraphics[width=\linewidth]{images/qmul_example_new.pdf}
\caption{Sample images from QMUL-SurvFace~\cite{cheng2018surveillance} dataset.} \label{fig:qmul_example}
\end{figure}
To our knowledge, this is the largest surveillance face recognition dataset. The face resolution ranges from 6/5 to 124/106 pixels in height/width, with an average of 24/20. Given LR facial appearance, surveillance FR may be less sensitive to the nationality than HR web FR. Among all identities, $\sim$10K are used for test purposes only, while the others are used for the training. We used the dataset for test purposes only. Specifically, we tested our models on the two protocols indicated into the dataset instructions, i.e. 1:1 face verification and 1:N face identification (open-set). 

